Sharp analysis of EM for learning mixtures of pairwise differences

We consider a symmetric mixture of linear regressions with random samples from the pairwise comparison design, which can be seen as a noisy version of a type of Euclidean distance geometry problem. We analyze the expectation-maximization (EM) algorithm locally around the ground truth and establish that the sequence converges linearly, providing an $\ell_\infty$-norm guarantee on the estimation error of the iterates. Furthermore, we show that the limit of the EM sequence achieves the sharp rate of estimation in the $\ell_2$-norm, matching the information-theoretically optimal constant. We also argue through simulation that convergence from a random initialization is much more delicate in this setting, and does not appear to occur in general. Our results show that the EM algorithm can exhibit several unique behaviors when the covariate distribution is suitably structured.

==> mixture_of_ranking_models.tex <==
\section{Introduction}
Mixtures of linear regressions are often used to model heterogeneous populations and have been widely studied in recent years \cite{}.
However, theoretical results in existing works are mostly restricted to Gaussian covariates.
In many areas such as \cite{}, measurements are often taken as pairwise comparisons between entities.
To study the pairwise-comparison design, we consider the following model of a symmetric mixture of two linear regressions with parameter vectors $\theta^*, - \theta^* \in \R^d$.
For $r = 1, \dots, N$, suppose that we observe $(x_r, y_r) \in \R^d \times \R$ satisfying 
\begin{align}\label{eq:model_symmetric}
y_r = z_r \, x_r^\top \theta^* + \epsilon_r , 
\end{align}
%where we observe $(x_r, y_r) \in \R^d \times \R$ for $r = 1, \dots, N$ and aim to estimate $\theta^* \in \R^d$. 
where
\begin{itemize} 
\item
the covariates $x_r$ follow the pairwise-comparison design:
$x_r = e_{i_r}-e_{j_r}$ for $i_r, j_r \in [d] := \{1,\dots,d\}$, where $e_i$ is the $i$th standard basis vector in $\R^d$;

\item
$z_r \in \{-1, 1\}$ is a latent sign indicating whether the observation is from component $\theta^*$ or $-\theta^*$;

\item
$\epsilon_r$ is the noise, which is assumed to be i.i.d.\ Gaussian for theoretical results.
\end{itemize}
Our goal is to estimate the parameter vector $\theta^* \in \R^d$.
%This model has been broadly studied in the literature, especially in the case where $x_r$ is Gaussian.

Other than understanding \eqref{eq:model_symmetric} as a mixture of linear regressions, we can reformulate it as follows in view of its natural connection to the Euclidean distance geometry problem and phase retrieval.
Let $y'_r = |y_r|$ be the observation and $\eps'_r = z_r \eps_r$ be the noise.
Because the sign $z_r$ is unobserved, model \eqref{eq:model_symmetric} is equivalent to 
\begin{align}\label{eq:model_abs}
y'_r = |x_r^\top \theta^* + \eps'_r|. 
\end{align}
Since $x_r = e_{i_r} - e_{j_r}$, we observe $|\theta^*_{i_r} - \theta^*_{j_r} + \eps'_r|$ which is the distance between two parameters contaminated by noise\footnote{It is more natural to have the noise $\eps'_r$ inside the absolute value because the distance is nonnegative.}.
Hence our goal is to reconstruct $\theta^*_1, \dots, \theta^*_d$ from pairwise distances, which is a noisy version of the classical distance geometry problem \cite{}.
More generally, \eqref{eq:model_abs} is the real-valued phase retrieval problem with noise \cite{}, where the covariates $x_r$ can take other form.

\subsection{The EM algorithm and our contributions}
The Expectation-Maximization (EM) algorithm has long been used for estimation in mixture models \cite{} and, particularly, in mixtures of linear regression \cite{}.
For Gaussian covariates $x_r$ in \eqref{eq:model_symmetric}, local linear convergence of the EM algorithm has been established in \cite{} and global convergence has been analyzed in \cite{}.
There is a large literature on the EM and other iterative algorithms for mixture of regressions; see, for example, \cite{} and references therein.
In this work, we apply the EM algorithm to model \eqref{eq:model_symmetric} and establish its local linear convergence around the ground truth $\theta^*$.
Moreover, we provide a sharp bound on the error achieved by the EM fixed point in estimating $\theta^*$.

Despite the extensive study of the EM algorithm for mixture models, our results differ from existing works in several crucial ways.
First, we show that the EM algorithm contracts in the $\ell_\infty$-norm, not the $\ell_2$-norm.
Second, we do not assume that each iterate of the EM algorithm takes in a fresh sample, and our convergence guarantee is not based on sample-splitting.
Third, a popular approach to analyzing the EM algorithm is through analyzing the population version of the algorithm first and then bounding the difference between the population iterates and the finite-sample iterates; on the other hand, we directly analyze the finite-sample EM algorithm.



\subsection{Organization}

\subsection{Notation} \label{sec:notation}
Let $d$ and $N$ be positive integers such that $3 \le d \le N$ throughout the paper. 
Define $[d] := \{1,\dots,d\}$ and $\binom{[d]}{2} := \{(i,j) : i,j \in [d], \, i<j\}$. 
Let $\bone$ denote the all-ones vector in $\R^d$, and let $\cH$ denote the orthogonal complement of $\bone$ in $\R^d$.

\section{Main results}
For the theoretical results to follow, we consider model \eqref{eq:model_symmetric} with the following assumptions.
First, the covariates are $x_r = e_{i_r}-e_{j_r}$ where $(i_r, j_r)_{r=1}^N$ are i.i.d.\ and uniformly random in $$\binom{[d]}{2} := \{(i,j) : i,j \in [d], \, i<j\}.$$ 
In other words, the comparisons are chosen randomly among all pairs of indices.
Second, the noise terms $(\epsilon_r)_{r=1}^N$ are i.i.d.\ $\cN(0,\sigma^2)$ and independent from the covariates.
Third, note that model \eqref{eq:model_symmetric} is invariant under any constant shift of $\theta^*$:
If $\theta^*$ is replaced by $\theta^* + c\,\mathbf{1}$ for a constant $c \in \R$, the response $y_r$ stays the same. Therefore, throughout the paper, we may assume that $\mathbf{1}^\top \theta^* = 0$, that is, $\theta^* \in \cH$ where $\cH$ is the orthogonal complement of the all-ones vector $\bone$ in $\R^d$.



%\begin{lemma}
%Suppose that $(x_r)_{r=1}^N$ are i.i.d.\ from the uniform distribution over $\{ e_i - e_j : (i,j) \in \binom{[d]}{2} \}$.
%Fix $\Delta > 0$ and define
%\(s_1  :=  |\{j \in [d] \, : \,|\theta_1^\ast - \theta_j^\ast| \leq \Delta\}|.\)
%There is an absolute constant $C>0$ such that for any $\delta \in (0,1)$, it holds with probability at least $1 - $ that
%$$
%\sum_{r = 1}^N \sum_{j=2}^d \bbone \big\{ x_r = e_1 - e_j , \, |\theta^*_1 - \theta^*_j| \le \Delta \big\}
%$$
%\end{lemma}
%
%\begin{proof}
%Define $Z_r := \sum_{j=2}^d \bbone \big\{ x_r = e_1 - e_j , \, |\theta^*_1 - \theta^*_j| \le \Delta \big\}$.
%It is easily seen that $Z_r \sim \Ber \big( \frac{2 s_1}{d(d-1)} \big)$
%\end{proof}


Define the sample covariance matrix of the covariates to be
\begin{equation}
\hat \Sigma := \frac{d-1}{2N} \sum_{r = 1}^N x_r x_r^\top.
\label{eq:def-samp-cov}
\end{equation}
%Recall that $\bone$ denotes the all-ones vector in $\R^d$ and $\cH$ denotes the orthogonal complement of $\bone$.
Note that $\bone$ is in the kernel of $\hat \Sigma$ and $\cH$ is an invariant subspace of $\hat \Sigma$.
Therefore, $\hat \Sigma$ can be viewed as a linear map on $\cH$.
Let $\hat \Sigma^\dag$ denote the pseudoinverse of $\hat \Sigma$; it is the true inverse of $\hat \Sigma$ if $\hat \Sigma$ is restricted to $\cH$ and is invertible.
Moreover, the normalization $\frac{d-1}{2N}$ is chosen so that \notecm{complete this}
$$
\E[\hat \Sigma] = 
$$

For $\theta \in \cH$, it is well-known \cite{} that the Easy-EM operator and the EM operator are defined respectively by
\begin{subequations} \label{eq:qq}
\begin{align}
\bar Q(\theta) &:= \frac{d-1}{2N} \sum_{r=1}^N \tanh \Big( \frac{ y_r \, x_r^\top \theta }{\sigma^2} \Big) y_r x_r, \label{eq:qq-1} \\
\hat Q(\theta)  &:=  \hat \Sigma^\dag \bar Q(\theta).
\label{eq:qq-2}
\end{align}
\end{subequations}
Therefore, starting from an initialization $\theta^{(0)}$, the EM iteration is
\begin{equation}
\theta^{(t+1)} := \hat Q( \theta^{(t)} ) = \left(\sum_{r=1}^Nx_rx_r^\top\right)^\dag  \sum_{r=1}^N \tanh \Big( \frac{ y_r \, x_r^\top \theta^{(t)} }{\sigma^2} \Big) y_r x_r , \qquad t \ge 0.
\label{eq:iteration-em}
\end{equation}

To facilitate the discussion of our main results, it is helpful to consider the following special class of parameter vectors $\theta^*$.
This type of assumption has also appeared in, for example, \cite{}.
Our results are more general \notecm{complete and discuss; introduce the running example $\theta_i = i/d + c$}

Our first result shows that the EM sequence $\{\theta^{(t)}\}_{t \ge 0}$ converges linearly to a limit $\hat \theta$ around the ground truth $\theta^*$ in the $\ell_\infty$-norm with high probability.
\notecm{currently the following theorem is Proposition~\ref{prop:em-contraction}. Going to simplify it.}

\begin{theorem}
\label{thm:em-contraction}
There exist absolute constants $C, C' > 0$ such that the following holds for any $\delta \in (0,1)$ and any integer $L \ge 2$.
Fix $\theta^{(0)} \in \cH$ and let $\Delta^{(0)} := \max\{ 4L \|\theta^{(0)} - \theta^*\|_\infty, 6 \sqrt{L} \, \sigma \}$. 
Suppose that
$$
N \ge C \max \Big\{ L^2 d^{\frac{L}{L-1}} \log \frac{dL}{\delta} , L^3 d \log \frac{L}{\delta} \Big\} , \qquad
\max_{i \in [d]} |S_i(\Delta^{(0)})| \le \frac{d}{C L^2} ,
$$
where 
$$
S_i(\Delta) := \{j \in [d] \setminus \{i\} : |\theta_i^* - \theta_j^*| \leq \Delta\}.
$$
Let $\{\theta^{(t)}\}_{t \ge 0}$ be the EM iterates defined in \eqref{eq:iteration-em}. 
Moreover, let 
$$
\tau := C' \sigma \sqrt{\frac{L\,d}{N}\log\frac d\delta} , \qquad
T := \max\bigg\{ 0, \bigg\lceil \log_{4/3} \bigg( \frac{\|\theta^{(0)} - \theta^*\|_\infty}{4\tau} \bigg) \bigg\rceil \bigg\} . 
$$
Then it holds with probability at least $1-\delta$ that 
\begin{itemize}
\item
there exists $\hat \theta \in \cH$ such that $\hat Q(\hat \theta) = \hat \theta$ and $\|\hat \theta - \theta^*\|_\infty \le 4 \tau$;
%i.e., $\hat \theta$ is a fixed point of $\hat Q$;

\item
the sequence $\{\theta^{(t)}\}_{t \ge 0}$ converges to $\hat \theta$;

\item
$\| \theta^{(T+t)} - \hat \theta \, \|_\infty \le 8 \tau / 2^t$ for all $t \ge 0$.
\end{itemize}
\end{theorem}

A more precise version of the above theorem is Proposition~\ref{prop:em-contraction}.
\notecm{discuss it}

Furthermore, we show that the limit $\hat \theta$ of the EM sequence achieves a sharp estimation error in the $\ell_2$-norm with high probability in the low-noise regime.

\begin{theorem}\label{thm:asymptotics}
There exist absolute constants $C, C' > 0$ such that the following holds for any $\delta \in (0,1)$ and any integer $L \ge 2$.
Fix $\theta^{(0)} \in \cH$ and let $\Delta^{(0)} := \max\{ 4L \|\theta^{(0)} - \theta^*\|_\infty, 6 \sqrt{L} \, \sigma \}$. 
Also, let $\Delta := 2 C \sigma \sqrt{\log \frac{N}{\delta}}$. 
Suppose that
\begin{equation}
N \ge C \max \Big\{ L^2 d^{\frac{L}{L-1}} \log \frac{dL}{\delta} , L^3 d \log \frac{L}{\delta} \Big\} , \qquad
N \gg L d  \log\frac d\delta \left(\log \frac{N}{\delta}\right)^3 ,
\label{eq:condition-N}
\end{equation}
and
\begin{equation}
\max_{i \in [d]} |S_i(\Delta^{(0)})| \le \frac{d}{C L^2} , \qquad
\max_{i \in [d]} |S_i(\Delta)| = o\left( \frac{d}{\log(N/\delta)} \right) ,
\label{eq:condition-Delta}
\end{equation}
where $S_i(\cdot)$ is defined in \eqref{def:S_i}. 
Let $\hat \theta$ be the limit of the EM sequence $\{\theta^{(t)}\}_{t \ge 0}$ defined in \eqref{eq:iteration-em} as guaranteed by Proposition~\ref{prop:sigma-dag-bound}. 
Then we have 
%Let $\hat\theta = \hat{Q}(\hat\theta)$ and $\theta^*$ be the true parameter. 
%We have
%\[(\hat{\Sigma} - A)(\hat\theta-\theta^*) = \bar Q(\theta^*) - \hat\Sigma\theta^* + \err.\]%\hat{G}(\theta^*) - \hat{\Sigma}\theta^* + \omega,\]
%Here, $\err \in \R^d$ such that
%\[\|\err\|_\infty \leq C'\,\frac{\sigma\,L\,d}{N}\log\frac d\delta\,\left(\log \frac{N}{\delta}\right)^{3/2},\]
%with probability at least $1 - 3\delta$, and $A$ is given by \eqref{eq:def-A}. 
% Furthermore, there exists an absolute constant $C > 0$ such that, for $\delta \in (0, 1)$ we have
% \[|\omega_i| \leq C\,\sigma\left(\frac{d}{N}\log\frac{d}{\delta}\right)\,\left(\log\frac{N}{\delta}\right)^{3/2},\]
% for all $i$ with probability at least $1 - \delta$.
$$
\hat \theta - \theta^* = \hat Q(\theta^*) - \theta^* + \err , 
$$
where $\|\err\|_\infty = o(\|\hat \theta - \theta^*\|_\infty)$. 
Furthermore, 
$$
\|\hat \theta - \theta^*\|_2^2 \le \sigma^2 \frac{d-1}{2N} \tr(\hat \Sigma^\dag) + C' \sigma^2 \left( \frac{d^{3/2}}{N}\sqrt{\log\frac{1}{\delta}}+ \frac{d}{N} \log \frac{1}{\delta} \right) .
$$
\end{theorem}

Note that the first term in the error is equal to 
$$
\sigma^2 \tr\bigg( \Big( \sum_{r=1}^N x_r x_r^\top \Big)^\dag \bigg) ,
$$
which is the optimal rate even for linear regression with no mixture. 
It is of order $\sigma^2 d^2/N$ and thus dominates the other terms. 
As a consequence, we have obtained a sharp $\ell_2$-norm bound.

\notecm{In the running example $\theta_i = i/d + c$, we have $S_i(\Delta) \asymp \Delta d$. Therefore, the hidden condition in \eqref{eq:condition-Delta} is that $\sigma$ needs to be polylogarithmically small.}

\notecm{A CLT type of result may be stated here, or better put in the following discussion section.}


\section{Further discussion}

There are several restrictions of our model and results admittedly.
For example, we have assumed a symmetric mixture of two linear regressions.
Moreover, our convergence guarantee of the EM algorithm is local in nature and may require an initialization in practice.
%We also impose a condition on the signal-to-noise ratio \ref{}.
Another natural question is how the EM algorithm compares to other algorithms such as spectral methods.
In this section, we discuss these points together with some possible extensions (in less rigorous terms).

\subsection{General mixtures of linear regressions}
One may consider the more general mixture of two linear regressions 
\begin{align}\label{ranking_model_original}
y_r = x_r^\top \theta^{[\ell_r]} + \epsilon_r,
\end{align}
where $\theta^{[1]},\, \theta^{[2]} \in \R^d$ and $(\ell_r)_{r=1}^N$ are i.i.d.\ and uniformly random over $\{1,2\}$. 
It is not difficult to estimate $\theta^{[1]} + \theta^{[2]}$ and center \eqref{ranking_model_original} to reduce it to \eqref{eq:model_symmetric}, up to a negligible error.

%In the following subsections, we will describe an iterative algorithm with an initialization procedure that recovers $\theta$ efficiently.

% Note the following:
% \begin{align*}
%     \EE[xx^\top] &= \frac{1}{d(d-1)}\sum_{j \not = k}(e_j-e_k)(e_j-e_k)^\top \\
%     &= \frac{2}{d(d-1)}\left(dI - \mathbf{1}\mathbf{1}^\top\right).
% \end{align*}
% So, we have that
% \[M  :=  \frac{d-1}{2}\EE[xx^\top] = I - \frac{\mathbf{1}\mathbf{1}^\top}{d}.\]
% We can now think of $M$ as the projection onto the vector-space $\mathbf{1}^\perp$.

\paragraph{Non-identifiability for mixtures with three or more components}
Suppose that there is an equally weighted mixture of $k$ components $\theta^{(1)}, \dots, \theta^{(k)} \in \R^d$ to be learned.
Consider the pairwise comparison design $x = e_i - e_j$ for $i, j \in [d]$.
%\paragraph{Linear model with three or more components}
%We turn to a $k$-mixture of linear models and 
We show that it is not identifiable if $k \ge 3$.
It suffices to give an example for $k = 3$.
Let
$$
\theta^{(1)} =
\begin{bmatrix}
1 \\ 2 \\ \theta_3 \\ \vdots \\ \theta_d
\end{bmatrix}
, \quad
\theta^{(2)} =
\begin{bmatrix}
3 \\ 3 \\ \theta_3 \\ \vdots \\ \theta_d
\end{bmatrix}
, \quad
\theta^{(3)} =
\begin{bmatrix}
2 \\ 4 \\ \theta_3 \\ \vdots \\ \theta_d
\end{bmatrix}
, \quad
\tilde{\theta}^{(1)} =
\begin{bmatrix}
2 \\ 2 \\ \theta_3 \\ \vdots \\ \theta_d
\end{bmatrix}
, \quad
\tilde{\theta}^{(2)} =
\begin{bmatrix}
1 \\ 3 \\ \theta_3 \\ \vdots \\ \theta_d
\end{bmatrix}
, \quad
\tilde{\theta}^{(3)} =
\begin{bmatrix}
3 \\ 4 \\ \theta_3 \\ \vdots \\ \theta_d
\end{bmatrix}
,
$$
where the unspecified entries $\theta_3, \dots, \theta_d$ can take any values.
It is not hard to see that, even if we observe the sets 
$$
\Big\{ \theta^{(\ell)}_i - \theta^{(\ell)}_j : \ell = 1,2,3 \Big\} \quad \text{ for all } (i, j) \in \binom{[d]}{2}
$$
with no noise, both mixtures $\{ \theta^{(\ell)} : \ell = 1,2,3 \}$ and $\{ \tilde \theta^{(\ell)} : \ell = 1,2,3 \}$ give the same sets of observations.
\notecm{Is the linear model with two unequally weighted components identifiable?}


\subsection{Divergence of the EM algorithm}
\notecm{numerical experiments show global convergence doesn't hold, and no convergence in the large-noise regime}


\subsection{Spectral method}
\notecm{worse than EM in the (low-noise) incomplete case, but can be used as initialization}


\begin{comment}
It remains to define an initial guess for $\theta^\ast$. Let $i,j$ be such that $|y_{ij}|$ is maximized. Without loss of generality, let $y_{ij} < 0$. We define $\tilde{\theta}$ as follows:
\[\tilde{\theta}_k = \left\{\begin{array}{cc}
0 & k = i \\
|y_{ij}| & k = j \\
|y_{ik}| & |y_{ik}| + |y_{kj}| \leq |y_{ij}| \\
-|y_{ik}| & |y_{ik}| + |y_{kj}| > |y_{ij}| \,,\, |y_{ik}| < |y_{kj}| \\
|y_{ij}| + |y_{ik}| & |y_{ik}| + |y_{kj}| > |y_{ij}| \,,\, |y_{ik}| \geq |y_{kj}| \\
\end{array}\right.\]
Finally, we let $\theta^{(0)} = \tilde{\theta} - (\sum_j\tilde{\theta}_j)\mathbf 1$.
\end{comment}

\subsection{Binary response}

\notecm{binary/logistic model}

\begin{comment}
\paragraph{Binary response}
Let us first show that, for the pairwise comparison design, a mixture of generalized linear models with binary response is not identifiable.
Suppose that we are given binary observations with mean $F(\theta^{(\ell)}_i - \theta^{(\ell)}_j)$ for a known link function $F$, where $i$ and $j$ are observed while $\ell$ is not.
In the infinite-sample limit, the full information we observe is
%the matrix
%$$
%\frac 1k \sum_{\ell=1}^k F \Big( \theta^{(\ell)} \bone^\top - \bone (\theta^{(\ell)})^\top \Big)
%$$
$$
\bigg\{ \frac 1k \sum_{\ell=1}^k F \Big( \theta^{(\ell)}_i - \theta^{(\ell)}_j \Big) \bigg\}_{i, j \in [d]} .
$$
\ notecm{I think the model is not identifiable. How can we show it? Note that if $F$ is the identity, this is trivial, because we only observe $\big( \frac 1k \sum_{\ell=1}^k \theta^{(\ell)} \big)_i - \big( \frac 1k \sum_{\ell=1}^k \theta^{(\ell)} \big)_j$.}
\end{comment}

\section{TBD}
\notecm{may provide a proof sketch of the zero-noise case: EM becomes alternating minimization}



%\[\err = \frac{d-1}{2N}\sum_{r = 1}^N\omega(\hat\theta, r, t_r)y_rx_r.\]
% To assist with the remainder of the proof and for simplicity of notation, we define
% \[\gamma(\mu, \sigma) = \EE_{X\sim \mathcal{N}(\mu, \sigma)}\left[\frac{X^2}{\sigma^2}\tanh'\left(\frac{X\mu}{\sigma^2}\right)\right].\]
% It follows that $\EE[A] = \Gamma$, where
% \[\Gamma_{ij} = \left\{\begin{array}{cc}
%     \frac{1}{d}\sum_{k \neq i}\gamma(\theta_i - \theta_k, \sigma) & i = j \\
%     -\frac{1}{d}\,\gamma(\theta_i - \theta_j, \sigma) & i \neq j.
% \end{array}\right.\]
% We also have $\EE[\hat{\Sigma}] = I - \frac{1}{d}\mathbf{1}\mathbf{1}^\top$.

%Let us now consider the error term $\omega(\hat\theta, t)$. 
%%Consequently, we have
%%\[\err = \frac{d-1}{2N}\sum_{r = 1}^N\omega(\hat\theta,r,t_r)y_rx_r = \omega(\hat \theta,t),\]
%%where $t \in \R^N$ such that $t_r = t_r$.
%From Lemma \ref{lem:taylor_error}, we have
%\[
%\|\omega(\hat\theta,t)\|_\infty 
%\le \frac{C'}{\sigma} \|\theta - \theta^*\|_\infty^2 \Big(\log \frac{N}{\delta}\Big)^{3/2} 
%%\leq \frac{48\|\theta - \theta^*\|_\infty^2}{\sigma}\max\left\{\left(\frac{\sigma}{\xi}\right)^3, \left(\frac{\xi}{\sigma}\right)^3\right\},
%\]
%with probability at least $1-\delta$ for $\xi\geq \max\{4\|\hat\theta - \theta^*\|_\infty, \|\eps\|_\infty\}$.
%From standard sub-Gaussian tail bounds, we can show for some absolute constant $C_1 > 0$,
%\[\|\eps\|_\infty \leq C_1\sigma\sqrt{\log\frac{N}{\delta}},\]
%with probability at least $1 - \delta$. Furthermore, from Lemma \ref{lem:em_true_dist}, we have for some absolute constant $C_2 > 0$,
%\[\|\hat\theta - \theta^*\|_\infty \leq C_2\sigma \sqrt{\frac{L\,d}{N}\log\frac d\delta},\]
%with probability at least $1 - \delta$.
%It follows for $\xi = C_1\sigma\sqrt{\log\frac{N}{\delta}}$, we have for some absolute constant $C'>0$
%\[\|\err\|_\infty \leq C'\,\frac{\sigma\,L\,d}{N}\log\frac d\delta\,\left(\log \frac{N}{\delta}\right)^{3/2},\]
%with probability at least $1 - 3\delta$.
%\end{proof}



%\begin{lemma}
%For $Z \sim \cN(0, 1)$ and constants $\alpha, \beta \in \R$, we have
%$$
%\E[ \tanh(\alpha + \beta Z) ]
%= , \qquad
%\E[ Z \tanh(\alpha + \beta Z) ]
%= .
%$$
%\end{lemma}
%
%\begin{proof}
%By Stein's lemma, we have
%$$
%\E[ Z \tanh(\alpha + \beta Z) ]
%= \beta \E \Big[ \frac{1}{\cosh^2 (\alpha + \beta Z)} \Big]
%=
%$$
%\end{proof}


\begin{comment}
\subsection{An alternative observation model}

Suppose that for $i, j \in [d]$, we have
$$
\tilde Y_{ij} =
\begin{cases}
z_{ij} (\theta^*_i - \theta^*_j) + \eps_{ij} \quad \text{ with probability } p & \text{ if } i < j , \\
\star \quad \text{ with probability } 1-p & \text{ if } i < j , \\
Y_{ji} & \text{ if } i > j , \\
0 & \text{ if } i = j ,
\end{cases}
$$
where $z_{ij}$ are uniform over $\{ \pm 1 \}$, $\eps_{ij}$ are independent zero-mean noise, and $\star$ means an entry missing with probability $1-p$ independently.
Define
$$
Y_{ij} =
\begin{cases}
\frac{1}{p} \tilde Y_{ij} & \text{ if } \tilde Y_{ij} \ne \star , \\
0 &  \text{ if } \tilde Y_{ij} = \star .
\end{cases}
$$
Then we have
$$
\E[ Y_{ij} \mid z_{ij} ] =
\begin{cases}
z_{ij} (\theta^*_i - \theta^*_j) & \text{ if } i \ne j , \\
0 &  \text{ if } i = j .
\end{cases}
$$
\end{comment}



\begin{comment}
\subsection{EM}

Let $\theta'$ be the resulting update from a single EM iteration on $\theta$. I.e.,
\[\theta'  :=  \left(\frac1n\sum_{r=1}^n x_rx_r^\top\right)^\dag\left(\frac1n \sum_{r=1}^n\tanh{\left(\frac{y_rx_r^\top\theta}{\sigma^2}\right)}y_rx_r\right).\]
The goal is to show $\|\theta'-\theta^*\|_{\infty} \leq \kappa \|\theta-\theta^*\|_\infty$ for some $\kappa < 1$. Recall that the consistency property guarantees
\[\mu = \EE_{X\sim \mathcal{N}(\mu, \sigma^2)}\left[X\tanh{\left(\frac{X\mu}{\sigma^2}\right)}\right].\]
It follows for each $r = 1,\ldots, n$,
\[\EE_{y_r\sim \mathcal{N}(x_r^\top\theta^*, \sigma^2)}\left[\tanh{\left(\frac{y_rx_r^\top\theta^*}{\sigma^2}\right)}y_rx_r\right] = x_rx_r^\top\theta^*.\]
This allows us to rewrite the difference $\theta'-\theta^*$ as follows
\begin{align*}
&~\theta' -\theta^* \\
&= \left(\frac1n\sum_{r=1}^n x_rx_r^\top\right)^\dag\left(\frac1n \sum_{r=1}^n\tanh{\left(\frac{y_rx_r^\top\theta}{\sigma^2}\right)}y_rx_r - \frac1n \sum_{r=1}^n\EE_{y_r\sim \mathcal{N}(x_r^\top\theta^*, \sigma^2)}\left[\tanh{\left(\frac{y_rx_r^\top\theta^*}{\sigma^2}\right)}y_rx_r\right]\right) \\
&= \underbrace{\left(\frac1n\sum_{r=1}^n x_rx_r^\top\right)^\dag}_{\mathbf A}
\underbrace{\left(\frac1n \sum_{r=1}^n\tanh{\left(\frac{y_rx_r^\top\theta}{\sigma^2}\right)}y_rx_r - \frac1n \sum_{r=1}^n\EE_{y_r\sim \mathcal{N}(x_r^\top\theta, \sigma^2)}\left[\tanh{\left(\frac{y_rx_r^\top\theta}{\sigma^2}\right)}y_rx_r\right]\right)}_{\mathbf B} \\
&\quad+ \underbrace{\left(\frac1n\sum_{r=1}^n x_rx_r^\top\right)^\dag\left(\frac1n \sum_{r=1}^n\EE_{y_r\sim \mathcal{N}(x_r^\top\theta, \sigma^2)}\left[\tanh{\left(\frac{y_rx_r^\top\theta}{\sigma^2}\right)}y_rx_r\right] - \frac1n \sum_{r=1}^n\EE_{y_r\sim \mathcal{N}(x_r^\top\theta^*, \sigma^2)}\left[\tanh{\left(\frac{y_rx_r^\top\theta^*}{\sigma^2}\right)}y_rx_r\right]\right)}_{\mathbf C}.
\end{align*}

% We can concentrate $\mathbf A$ using standard concentration results and the fact that $\|M\|_\infty \leq \|M\|_2$ for any matrix $M$.
In the following lemma, we provide a bound for $\mathbf B$.

\begin{lemma}
With probability at least $1 - \ldots$, we have
\[\left\|\frac1n \sum_{r=1}^n\left(\tanh{\left(\frac{y_rx_r^\top\theta}{\sigma^2}\right)}y_rx_r - \EE_{y_r\sim \mathcal{N}(x_r^\top\theta, \sigma^2)}\left[\tanh{\left(\frac{y_rx_r^\top\theta}{\sigma^2}\right)}y_rx_r\right]\right)\right\|_\infty \leq t.\]
\end{lemma}

\begin{proof}

Let $v \in \R^d$. We define the following function $f_v\,:\,\R^n \to \R$
\[f_v(y) = \frac1n \sum_{r=1}^n\tanh{\left(\frac{y_rx_r^\top\theta}{\sigma^2}\right)}y_rx_r^\top v.\]


\end{proof}
\end{comment}






\begin{comment}

\begin{lemma}[Chernoff's inequality]
\label{lem:chernoff}
Let $X_i$ be independent Bernoulli random variables with parameters $p_i \in [0,1]$ for $i \in [N]$.
Let $\mu := \sum_{i=1}^N p_i$.
Then for any $t > \mu$, we have
$$
\p \bigg\{ \sum_{i=1}^N X_i \ge t \bigg\} \le e^{-\mu} (e \mu / t)^t ,
$$
and for any $t < \mu$, we have
$$
\p \bigg\{ \sum_{i=1}^N X_i \le t \bigg\} \le e^{-\mu} (e \mu / t)^t .
$$
\end{lemma}


\ notecm{old proofs in the appendix}

\section{Old proofs}

We first consider the noiseless case,
\[y = zx^\top\theta.\]
From our data, we can estimate $y_{ij} = \theta_i^\ast - \theta_j^\ast$. \adcomment{How do we have the estimates $y_{ij}$? I don't remember this procedure.}
We conduct the following iterative procedure for a well chosen $\theta^{(0)}$.
\begin{align}\label{update_step}
\theta^{(t+1)} = \frac{1}{d}\sum_{i,j=1}^d\sign\left(\left(\theta_i^{(t)} - \theta_j^{(t)}\right)y_{ij}\right)y_{ij}(e_i - e_j).
\end{align}
Note, for each coordinate in $\theta^{(t+1)}$, the update is as follows:
\[\theta_i^{(t+1)} = \frac{1}{d}\sum_{j=1}^d\sign\left(\left(\theta_i^{(t)} - \theta_j^{(t)}\right)y_{ij}\right)y_{ij}.\]
Furthermore, if $\theta^{(t)} = \theta^\ast$, then $\theta^{(t+1)} = \theta^\ast$.

In the following lemma, we show that the update in \ref{update_step} produces a better estimate for $\theta^\ast$.

\begin{lemma}\label{iteration_noiseless}
If $|\theta_i^{(t)} - \theta_i^\ast| \leq \Delta$ and $s_i \leq c\,d$ for all $i \in [d]$, then $|\theta_i^{(t+1)} - \theta_i^\ast| \leq 4\,c\,\Delta$.
\end{lemma}

\begin{proof}
Note that $\mathbf{1}^\top\theta^\ast = 0$. With that in mind, we have
\begin{align*}
\theta_i^{(t+1)} - \theta_i^\ast &= \frac{1}{d}\sum_{j=1}^d\sign\left(\left(\theta_i^{(t)} - \theta_j^{(t)}\right)\left(\theta_i^\ast - \theta_j^\ast\right)\right)\left(\theta_i^\ast - \theta_j^\ast\right) - \theta_i^\ast \\
&= \frac{1}{d}\sum_{j=1}^d\sign\left(\left(\theta_i^{(t)} - \theta_j^{(t)}\right)\left(\theta_i^\ast - \theta_j^\ast\right)\right)\left(\theta_i^\ast - \theta_j^\ast\right) - \frac{1}{d}\sum_{j=1}^d\left(\theta_i^\ast - \theta_j^\ast\right) \\
&= \frac{-2}{d}\sum_{j=1}^d\mathbbm{1}\left\{\sign\left(\left(\theta_i^{(t)} - \theta_j^{(t)}\right)\left(\theta_i^\ast - \theta_j^\ast\right)\right) = -1\right\}\left(\theta_i^\ast - \theta_j^\ast\right).
\end{align*}
Since $|\theta_k^{(t)} - \theta_k^\ast| \leq \Delta$ for all $k$, we have the following:
\[|\theta_i^\ast - \theta_j^\ast| > 2\Delta \implies \sign\left(\left(\theta_i^{(t)} - \theta_j^{(t)}\right)\left(\theta_i^\ast - \theta_j^\ast\right)\right) = 1.\]
With this in hand, we get the desired bound below:
\begin{align*}
|\theta_i^{(t+1)} - \theta_i^\ast| &\leq \frac{2}{d}\sum_{j=1}^d\mathbbm{1}\left\{\sign\left(\left(\theta_i^{(t)} - \theta_j^{(t)}\right)\left(\theta_i^\ast - \theta_j^\ast\right)\right) = -1\right\}|\theta_i^\ast - \theta_j^\ast| \\
&\leq \frac{2}{d}\cdot s_i\cdot 2\Delta \\
&\leq 4\,c\,\Delta.
\end{align*}
\end{proof}

Next, we consider the noisy case,
\[y = zx^\top\theta + \epsilon.\]
From our data, we can estimate $y_{ij} = \theta_i^\ast - \theta_j^\ast + \epsilon_{ij}$. \adcomment{Same as before.} We conduct the same procedure as in \ref{update_step}. We define a new parameter $s_i^{(t)}$ similar to before:
\[s_i^{(t)} :=  |\{j\,:\, \sign\left(\left(\theta_i^{(t)}-\theta_j^{(t)}\right)y_{ij}\right) = -1\}|.\]
Let $\Delta' = 2\Delta + C$ where $C$ is an upper-bound on $\epsilon_{ij}$ independent of $d$ and $\theta^\ast$. In the following lemma we show that $\theta^{(t+1)}$ is a better estimate for $\theta^\ast$.

\begin{lemma}\label{iteration_noisy}
If $|\theta_i^{(t)} - \theta_i^\ast| \leq \Delta'$ and $s_i \leq c\,d$, then $|\theta_i^{(t+1)} - \theta_i^\ast| \leq 4c\,\Delta' + 5C$.
\end{lemma}

\begin{proof}
Similar to the computation in Lemma \ref{iteration_noiseless}, we have the following:
\begin{align*}
\theta_i^{(t+1)} - \theta_i^\ast &= \frac{-2}{d}\sum_{j=1}^d\mathbbm{1}\left\{\sign\left(\left(\theta_i^{(t)} - \theta_j^{(t)}\right)y_{ij}\right) = -1\right\}\left(\theta_i^\ast - \theta_j^\ast\right) \\
&\qquad \frac{-2}{d}\sum_{j=1}^d\mathbbm{1}\left\{\sign\left(\left(\theta_i^{(t)} - \theta_j^{(t)}\right)y_{ij}\right) = -1\right\}\epsilon_{ij} \\
&\qquad + \frac{1}{d}\sum_{j = 1}^d\epsilon_{ij}.
\end{align*}
Note that if $\sign\left(\left(\theta_i^{(t)} - \theta_j^{(t)}\right)y_{ij}\right) = -1$, then $|\theta_i^\ast-\theta_j^\ast| \leq 2\Delta' + C$. With this in mind, we simplify the above to get:
\begin{align*}
|\theta_i^{(t+1)} - \theta_i^\ast| &\leq \frac{2s_i}{d}\left(2\Delta' + C + C\right) + C \\
&\leq 4c\,\Delta' + 5C.
\end{align*}
\end{proof}
In Lemma \ref{iteration_noiseless}, for small enough $c$, convergence is expected in $O(\log \Delta)$ iterations. Similarly, in Lemma \ref{iteration_noisy}, provided $C$ isn't too large, convergence is expected in $O(\log \Delta')$ iterations. It remains to find a $\theta^{(0)}$ and $\Delta$ such that we can apply the lemmas of this section.
\end{comment}





\begin{comment}

\subsection{Alternating minimization}

Suppose that we have independent observations
$$
y_r = z_r \, x_r^\top \theta^* + \epsilon_r , \qquad r = 1, \dots, N ,
$$
where $z_r$ is uniform over $\{\pm 1\}$, $x_r$ is uniform over $\{ e_i - e_j : (i, j) \in \binom{[d]}{2} \}$, and $\eps_r$ is noise.

\ notecm{fix conflation of notation $\theta^{(t)}$: an iterate or a component in the mixture}

Define the sign function
$$
\sign(t) =
\begin{cases}
1 & \text{ if } t \ge 0 ,\\
-1 & \text{ if } t < 0 .
\end{cases}
$$
Consider the following alternating minimization procedure motivated by least squares. Starting from $\theta^{(0)}$, for $t \ge 0$, we iteratively compute:
\begin{itemize}
\item
$z^{(t)}_r := \sign(y_r \, x_r^\top \theta^{(t)})$;

\item
$\theta^{(t+1)} := \frac{d-1}{2N} \sum_{r=1}^N z^{(t)}_r y_r x_r$.
\end{itemize}
In short, we have
\begin{equation}
\theta^{(t+1)} := \frac{d-1}{2N} \sum_{r=1}^N \sign(y_r \, x_r^\top \theta^{(t)}) y_r x_r.
\label{eq:iteration-am}
\end{equation}

\subsubsection{Analysis}

To analyze the iterate \eqref{eq:iteration-am}, we compare it to
\begin{equation}
\tilde \theta := \frac{d-1}{2N} \sum_{r=1}^N \sign(y_r \, x_r^\top \theta^*) y_r x_r ,
\label{eq:iteration-am-truth}
\end{equation}
that is, the one-step iterate from the ground-truth $\theta^*$.

For notational simplicity, let us consider iteration of the first entry $\theta^{(t)}_1$ of the parameter vector.
The same analysis applies to any other entry with straightforward modification.

\begin{lemma}
Suppose that $|\theta^{(t)}_j - \theta^*_j| \le \Delta$ for all $j \in [d]$ for a fixed $\Delta > 0$. Define
\begin{equation}
s_1  :=  \big|\big\{j \in [d] \setminus \{1\} : |\theta_1^\ast - \theta_j^\ast| \leq 2 \Delta\big\}\big|.
\label{eq:def-s1}
\end{equation}
Let $\|\eps\|_\infty := \max_{r \in [N]} |\eps_r|$.
Then there is an absolute constant $C>0$ such that for any $\delta \in (0,1)$,
\begin{equation*}
\big| \theta^{(t+1)}_1 - \tilde \theta_1 \big|
\le (2 \Delta + \|\eps\|_\infty) \bigg( \frac{2 s_1}{d}
+ C \sqrt{ \frac{s_1}{N} \log \frac{1}{\delta} }
+ C \frac{d}{N} \log \frac{1}{\delta}  \bigg)
\end{equation*}
with probability at least $1 - \delta$.
%For any $D>0$, there exists a constant $C > 0$ depending only on $D$ such that
%%the following holds.
%%If $d \ge C$ and $N \ge C d \log d$, then we have that with probability at least $1 - N^{-D}$,
%$$
%\big| \theta^{(t+1)}_1 - \tilde \theta_1 \big|
%\le (2 \Delta + \|\eps\|_\infty) \bigg( \frac{2 s_1}{d}
%+ C \sqrt{ \frac{s_1}{N} \log N }
%+ C \frac{d}{N} \log N \bigg)
%$$
%with probability at least $1 - N^{-D}$.
\end{lemma}

\ notecm{In the noiseless case, we have $\|\eps\|_\infty = 0$ and $\tilde \theta = \theta^*$. As long as $\Delta$ is small so that $s_1 \le d/10$ (which is a reasonable condition), then the bound is $\Delta/2$. Thus we get linear convergence.
However, in the noisy case, even $\tilde \theta_1$ is not close to $\theta^*_1$---see a remark below---so AM iteration simply doesn't work.}

\ notecm{I still hope such an analysis is useful. Let's consider EM (or some other iteration) instead of AM. Then I believe we should have $\tilde \theta_1 - \theta^*_1 \asymp \sigma \sqrt{d/N}$, where $\sigma$ is the max noise deviation and $\sigma \sqrt{d/N}$ is the optimal rate. (Starting from the ground truth should work once we choose the correct iteration.) Suppose that a bound of the above form holds: if $\big| \theta^{(t)}_1 - \theta^*_1 \big| \le \Delta$, then
$$
\big| \theta^{(t+1)}_1 - \theta^*_1 \big|
\le (2 \Delta + \sigma) ( 2 s_1/d + C \sqrt{s_1/N} + C d/N ) + C \sigma \sqrt{d/N} .
$$
Let's say $\theta^*_j \asymp j/d$ and $\Delta, \sigma \le 1/20$. Then $s_1 \asymp \Delta d$, so the bound becomes
$$
\big| \theta^{(t+1)}_1 - \theta^*_1 \big|
\le (2 \Delta + \sigma) ( 2 \Delta + C \sqrt{\Delta d/N} + C d/N ) + C \sigma \sqrt{d/N}
\le \Delta/2 + C_2 \sigma \sqrt{d/N} .
$$
Hence we get linear convergence up to the optimal rate. The condition $\Delta \le 1/20$ means a somewhat warm start; $\sigma \le 1/20$ means noise not too large. But since the signal is at most size $1$ with gaps $1/d$, I think these conditions are not unreasonable.
}

\begin{proof}
We can write the iteration of the first entry as
$$
\theta^{(t+1)}_1 = \frac{d-1}{2N} \sum_{r : x_r = e_1 - e_j} \sign \big( y_r (\theta^{(t)}_1 - \theta^{(t)}_j) \big) y_r ,
$$
where the sum is over all $r \in [N]$ for which $x_r = e_1 - e_j$ for any $j \in [d]$.
In other words, we use the shorthand
$$
\sum_{r : x_r = e_1 - e_j} \square_{r,j} := \sum_{r=1}^N \sum_{j=2}^d \bbone \{x_r = e_1 - e_j\} \cdot \square_{r,j} .
$$
Similarly, for $\tilde \theta$ defined in \eqref{eq:iteration-am-truth}, we have
$$
\tilde \theta_1 = \frac{d-1}{2N} \sum_{r : x_r = e_1 - e_j} \sign \big( y_r (\theta^*_1 - \theta^*_j) \big) y_r .
$$
It follows that
\begin{align}
\big| \theta^{(t+1)}_1 - \tilde \theta_1 \big|
&= \bigg| \frac{d-1}{2N} \sum_{r : x_r = e_1 - e_j} \Big[ \sign \big( y_r (\theta^{(t)}_1 - \theta^{(t)}_j) \big) - \sign \big( y_r (\theta^*_1 - \theta^*_j) \big) \Big] y_r \bigg| \notag \\
&\le \frac{d-1}{2N} \sum_{r : x_r = e_1 - e_j} \Big| \sign \big( \theta^{(t)}_1 - \theta^{(t)}_j \big) - \sign \big( \theta^*_1 - \theta^*_j \big) \Big| \cdot |y_r| . \label{eq:sign-sum}
\end{align}

%Therefore,
%\begin{align}
%\big| \theta^{(t+1)}_1 - \theta^*_1 \big|
%&\le \bigg| \frac{d-1}{2N} \bigg( \sum_{r : x_r = e_1 - e_j} (\theta^*_1 - \theta^*_j) \bigg) - \theta^*_1 \bigg|
%+ \frac{d-1}{2N} \, \bigg| \sum_{r : x_r = e_1 - e_j} \eps_r \bigg| \notag \\
%&\qquad + \frac{d-1}{N} \, \bigg| \sum_{r : x_r = e_1 - e_j} (\theta^*_1 - \theta^*_j + \eps_r) \, \bbone \big\{ y_r (\theta^{(t)}_1 - \theta^{(t)}_j) < 0 \big\} \bigg|
%\label{eq:3-terms}
%\end{align}

Consider $r \in [N]$ for which $x_r = e_1 - e_j$.
Recall that $|\theta^{(t)}_j - \theta^*_j| \le \Delta$ for all $j \in [d]$.
%Thus, if $\theta^*_1 - \theta^*_j > 2 \Delta$, then
%$$
%\theta^{(t)}_1 - \theta^{(t)}_j \ge \theta^*_1 - \theta^*_j - 2 \Delta > 0 .
%$$
%It follows that $\sign \big( \theta^{(t)}_1 - \theta^{(t)}_j \big) = \sign \big( \theta^*_1 - \theta^*_j \big)$.
%The same conclusion holds if $\theta^*_1 - \theta^*_j < - 2 \Delta$.
As a result, if $\sign \big( \theta^{(t)}_1 - \theta^{(t)}_j \big) \ne \sign \big( \theta^*_1 - \theta^*_j \big)$, then we must have $|\theta^*_1 - \theta^*_j| \le 2 \Delta$ and so
$$
|y_r| \le |\theta^*_1 - \theta^*_j| + |\eps_r|
\le 2 \Delta + \|\eps\|_\infty .
$$
Hence we obtain from \eqref{eq:sign-sum} that
\begin{equation}
\big| \theta^{(t+1)}_1 - \tilde \theta_1 \big|
\le \frac{d-1}{N} \sum_{r : x_r = e_1 - e_j} \bbone \big\{ |\theta^*_1 - \theta^*_j| \le 2 \Delta \big\} \cdot (2 \Delta + \|\eps\|_\infty) .
\label{eq:ind-sum}
\end{equation}

Furthermore, by the definition of $s_1$ in \eqref{eq:def-s1},
$$
\sum_{r : x_r = e_1 - e_j} \bbone \big\{ |\theta^*_1 - \theta^*_j| \le 2 \Delta \big\}
= \sum_{r=1}^N \sum_{j=2}^d \bbone \big\{ x_r = e_1 - e_j, |\theta^*_1 - \theta^*_j| \le 2 \Delta \big\}
\sim \Bin \Big( N, \frac{2 s_1}{d(d-1)} \Big) .
$$
By a standard binomial tail bound, there is an absolute constant $C_1 > 0$ such that for any $\delta > 0$,
$$
\sum_{r : x_r = e_1 - e_j} \bbone \big\{ |\theta^*_1 - \theta^*_j| \le 2 \Delta \big\}
\le \frac{2 N s_1}{d(d-1)}
+ C_1 \sqrt{ \frac{N s_1}{d (d-1)} \log \frac{1}{\delta} }
+ C_1 \log \frac{1}{\delta}
$$
with probability at least $1 - \delta$.
Combining this bound with \eqref{eq:ind-sum} yields the conclusion.
%Therefore, the conclusion follows by setting $\delta = N^{-D}$.
\end{proof}


\begin{lemma}
Then there is an absolute constant $C>0$ such that for any $\delta \in (0,1)$,
\begin{equation*}
\big| \tilde \theta_1 - \theta^*_1 \big|
\le
\end{equation*}
with probability at least $1 - \delta$.
\end{lemma}

\begin{proof}
%Since $\sum_{j=1}^d \theta^*_j = 0$, we have $\frac 1d \sum_{j=2}^d (\theta^*_1 - \theta^*_j) = \theta^*_1$.
%We have
%$$
%\tilde \theta_1 - \theta^*_1 = \frac{d-1}{2N} \sum_{r : x_r = e_1 - e_j} \sign \big( y_r (\theta^*_1 - \theta^*_j) \big) y_r .
%$$

We have
\begin{align*}
\tilde \theta_1
&= \frac{d-1}{2N} \sum_{r : x_r = e_1 - e_j} \sign \big( y_r (\theta^*_1 - \theta^*_j) \big) y_r \\
&= \frac{d-1}{2N} \bigg( \sum_{r : x_r = e_1 - e_j} (\theta^*_1 - \theta^*_j + \eps_r)
- 2 \sum_{r : x_r = e_1 - e_j} y_r \, \bbone \big\{ y_r (\theta^*_1 - \theta^*_j) < 0 \big\} \bigg) .
\end{align*}
Therefore,
\begin{align}
\big| \tilde \theta_1 - \theta^*_1 \big|
&\le \bigg| \Big( \frac{d-1}{2N} \sum_{r : x_r = e_1 - e_j} (\theta^*_1 - \theta^*_j) \Big) - \theta^*_1 \bigg|
+ \frac{d-1}{2N} \, \bigg| \sum_{r : x_r = e_1 - e_j} \eps_r \bigg| \notag \\
&\qquad + \frac{d-1}{N} \, \bigg| \sum_{r : x_r = e_1 - e_j} y_r \, \bbone \big\{ y_r (\theta^*_1 - \theta^*_j) < 0 \big\} \bigg| .
\label{eq:3-terms}
\end{align}
\ notecm{The first two terms can be controlled by the two lemmas below. However, the last term is unavoidable and can be large when the noise is larger than gaps. For example, if $\theta^*_1 - \theta^*_j$ are all positive but smaller than the noise deviation $\sigma$, then $y_r$ are negative and of size $\sigma$. The last term is thus of size $\sigma$, which is meaningless. This shows AM iteration doesn't work in the noisy case.}
\end{proof}


%\begin{lemma}
%Suppose that $|\theta^{(t)}_j - \theta^*_j| \le \Delta'$ for all $j \in [d]$ for a fixed $\Delta' > 0$.
%Fix a quantity
%$$
%\Delta \ge \max\{2 \Delta', \|\eps\|_\infty\}
%$$
%and define
%%\[s_i  :=  |\{j\,:\,|\theta_i^\ast - \theta_j^\ast| \leq 2\Delta\}|.\]
%\[s_1  :=  |\{j \in [d] \, : \, j \ne 1, \, |\theta_1^\ast - \theta_j^\ast| \leq \Delta\}|.\]
%
%For any $D>0$, there exists a constant $C > 0$ depending only on $D$ such that the following holds.
%If $d \ge C$ and $N \ge C d \log d$, then we have that with probability at least $1 - N^{-D}$,
%$$
%\big| \theta^{(t+1)}_1 - \theta^*_1 \big|
%\le C (\|\theta^*\|_\infty + \sigma) \sqrt{\frac{d}{N} \log N}
%+ \Delta \bigg( \frac{4 s_1}{d} + C \sqrt{ \frac{s_1}{N} \log N } + C \frac{d}{N} \log N \bigg) .
%$$
%\end{lemma}
%
%\ notecm{The requirement $\Delta \ge \|\eps\|_\infty$ is very bad and seems unavoidable according to analysis and simulation. However, in the noiseless case $\eps = 0$, the iteration works well and the proof is basically done.}
%
%\begin{proof}
%We can write the iteration of the first entry as
%%$$
%%\theta^{(t+1)}_i = \frac{d-1}{2N} \sum_{r : x_r = e_i - e_j} \sign \big( y_r (\theta^{(t)}_i - \theta^{(t)}_j) \big) y_r .
%%$$
%$$
%\theta^{(t+1)}_1 = \frac{d-1}{2N} \sum_{r : x_r = e_1 - e_j} \sign \big( y_r (\theta^{(t)}_1 - \theta^{(t)}_j) \big) y_r .
%$$
%It is not hard to see that
%\begin{align*}
%\theta^{(t+1)}_1
%%&= \frac{d-1}{2N} \sum_{r : x_r = e_1 - e_j} \sign \big( y_r (\theta^{(t)}_1 - \theta^{(t)}_j) \big) y_r \\
%&= \frac{d-1}{2N} \sum_{r : x_r = e_1 - e_j} \sign \big( y_r (\theta^{(t)}_1 - \theta^{(t)}_j) \big) (\theta^*_1 - \theta^*_j + \eps_r) \\
%%&= \frac{d-1}{2N} \bigg( \sum_{r : x_r = e_1 - e_j} (\theta^*_1 - \theta^*_j)
%%- 2 \sum_{r : x_r = e_1 - e_j} (\theta^*_1 - \theta^*_j) \, \bbone \big\{ y_r (\theta^{(t)}_1 - \theta^{(t)}_j) < 0 \big\}  \\
%%&\qquad \qquad \quad + \sum_{r : x_r = e_1 - e_j} \eps_r
%%- 2 \sum_{r : x_r = e_1 - e_j} \eps_r \, \bbone \big\{ y_r (\theta^{(t)}_1 - \theta^{(t)}_j) < 0 \big\} \bigg) .
%&= \frac{d-1}{2N} \bigg( \sum_{r : x_r = e_1 - e_j} (\theta^*_1 - \theta^*_j + \eps_r)
%- 2 \sum_{r : x_r = e_1 - e_j} (\theta^*_1 - \theta^*_j + \eps_r) \, \bbone \big\{ y_r (\theta^{(t)}_1 - \theta^{(t)}_j) < 0 \big\} \bigg) .
%\end{align*}
%Therefore,
%\begin{align}
%\big| \theta^{(t+1)}_1 - \theta^*_1 \big|
%&\le \bigg| \frac{d-1}{2N} \bigg( \sum_{r : x_r = e_1 - e_j} (\theta^*_1 - \theta^*_j) \bigg) - \theta^*_1 \bigg|
%+ \frac{d-1}{2N} \, \bigg| \sum_{r : x_r = e_1 - e_j} \eps_r \bigg| \notag \\
%&\qquad + \frac{d-1}{N} \, \bigg| \sum_{r : x_r = e_1 - e_j} (\theta^*_1 - \theta^*_j + \eps_r) \, \bbone \big\{ y_r (\theta^{(t)}_1 - \theta^{(t)}_j) < 0 \big\} \bigg|
%\label{eq:3-terms}
%\end{align}
%
%Consider $r \in [N]$ for which $x_r = e_1 - e_j$.
%If $\theta^*_1 - \theta^*_j > \Delta$, then
%$$
%y_r = \theta^*_1 - \theta^*_j + \eps_r > \Delta - |\eps_r| \ge 0 .
%$$
%In addition,
%$$
%\theta^{(t)}_1 - \theta^{(t)}_j \ge \theta^*_1 - \theta^*_j - 2 \Delta' \ge \Delta - 2 \Delta' \ge 0 .
%$$
%It follows that $y_r (\theta^{(t)}_1 - \theta^{(t)}_j) \ge 0$.
%Similarly, if $\theta^*_1 - \theta^*_j < - \Delta$, we again obtain $y_r (\theta^{(t)}_1 - \theta^{(t)}_j) \ge 0$.
%Therefore, if $y_r (\theta^{(t)}_1 - \theta^{(t)}_j) < 0$, then we must have $|\theta^*_1 - \theta^*_j| \le \Delta$.
%As a result,
%\begin{equation}
%\bigg| \sum_{r : x_r = e_1 - e_j} (\theta^*_1 - \theta^*_j) \, \bbone \big\{ y_r (\theta^{(t)}_1 - \theta^{(t)}_j) < 0 \big\} \bigg|
%\le \sum_{r : x_r = e_1 - e_j} \Delta \, \bbone \big\{ |\theta^*_1 - \theta^*_j| \le \Delta \big\}
%\label{eq:term-3}
%\end{equation}
%and
%\begin{equation}
%\bigg| \sum_{r : x_r = e_1 - e_j} \eps_r \, \bbone \big\{ y_r (\theta^{(t)}_1 - \theta^{(t)}_j) < 0 \big\} \bigg| \le \sum_{r : x_r = e_1 - e_j} \|\eps\|_\infty \, \bbone \big\{ |\theta^*_1 - \theta^*_j| \le \Delta \big\} .
%\label{eq:term-4}
%\end{equation}
%
%Moreover, note that
%$$
%\sum_{r : x_r = e_1 - e_j} \bbone \big\{ |\theta^*_1 - \theta^*_j| \le \Delta \big\}
%= \sum_{r=1}^N \bbone \big\{ x_r = e_1 - e_j, |\theta^*_1 - \theta^*_j| \le \Delta \big\}
%\sim \Bin \Big( N, \frac{2 s_1}{d(d-1)} \Big) .
%$$
%By a standard binomial tail bound, there is an absolute constant $C_1 > 0$ such that for any $\delta > 0$,
%$$
%\sum_{r : x_r = e_1 - e_j} \bbone \big\{ |\theta^*_1 - \theta^*_j| \le \Delta \big\}
%\le \frac{2 N s_1}{d(d-1)}
%%+ \frac{N}{8 \, d}
%+ C_1 \sqrt{ \frac{N s_1}{d (d-1)} \log \frac{1}{\delta} } + C_1 \log \frac{1}{\delta}
%$$
%with probability at least $1 - \delta$.
%Combining this bound with \eqref{eq:term-3} and \eqref{eq:term-4} yields
%\begin{equation}
%\bigg| \sum_{r : x_r = e_1 - e_j} (\theta^*_1 - \theta^*_j + \eps_r) \, \bbone \big\{ y_r (\theta^{(t)}_1 - \theta^{(t)}_j) < 0 \big\} \bigg|
%\le 2 \Delta \bigg( \frac{2 N s_1}{d(d-1)} + C_1 \sqrt{ \frac{N s_1}{d (d-1)} \log \frac{1}{\delta} } + C_1 \log \frac{1}{\delta} \bigg)
%\label{eq:terms-4-5}
%\end{equation}
%with probability at least $1 - \delta$, since $\Delta \ge \|\eps\|_\infty$.
%
%Finally, plugging \eqref{eq:terms-4-5} and the bounds from Lemmas~\ref{lem:theta-1-theta-j} and~\ref{lem:eps-r-conc} into \eqref{eq:3-terms}, we obtain
%\begin{align*}
%\big| \theta^{(t+1)}_1 - \theta^*_1 \big|
%&\le C_3 \|\theta^*\|_\infty \Big( \sqrt{\frac{d}{N} \log \frac{1}{\delta}} + \frac{d}{N} \log \frac{1}{\delta} \Big)
%+ C_3 \sigma \sqrt{\frac{d}{N} \log \frac{1}{\delta}} \\
%& \qquad + 2 \Delta \bigg( \frac{2 s_1}{d} + C_1 \sqrt{ \frac{s_1}{N} \log \frac{1}{\delta} } + C_1 \frac{d}{N} \log \frac{1}{\delta} \bigg)
%\end{align*}
%with probability at least $1 - \delta - \exp(-c_2 N/d)$, where $c_2, C_3>0$ are absolute constants.
%Therefore, the conclusion follows from setting $\delta = N^{-D}/2$.
%\end{proof}


\subsubsection{Lemmas to be used}

\begin{lemma}
\label{lem:theta-1-theta-j}
Suppose that $(x_r)_{r=1}^N$ are i.i.d.\ from the uniform distribution over $\{ e_i - e_j : (i,j) \in \binom{[d]}{2} \}$. Then there is an absolute constant $C>0$ such that for any $\delta \in (0,1)$, it holds with probability at least $1 - \delta$ that
$$
\bigg| \bigg( \frac{d-1}{2N} \sum_{r = 1}^N \sum_{j=2}^d (\theta^*_1 - \theta^*_j) \, \bbone \{ x_r = e_1 - e_j \} \bigg) - \theta^*_1 \bigg|
\le C \|\theta^*\|_\infty \Big( \sqrt{\frac{d}{N} \log \frac{1}{\delta}} + \frac{d}{N} \log \frac{1}{\delta} \Big) .
$$
\end{lemma}

\begin{proof}
Define $Z_r := \frac{d-1}{2} \sum_{j=2}^d (\theta^*_1 - \theta^*_j) \, \bbone \{ x_r = e_1 - e_j \}$. It suffices to apply Bernstein's inequality to bound $\big| \frac 1N \sum_{r=1}^N Z_ r - \theta^*_1 \big|$.
To this end, we first check that
$$
\E[Z_r]
= \frac{d-1}{2} \sum_{j=2}^d (\theta^*_1 - \theta^*_j) \, \frac{2}{d(d-1)}
= \theta^*_1
$$
since $\sum_{j=1}^d \theta^*_j = 0$.
Moreover, we have
$$
|Z_r|
%= \bigg| \frac{d-1}{2} \sum_{j=2}^d (\theta^*_1 - \theta^*_j) \, \bbone \{ x_r = e_1 - e_j \} \bigg|
\le \frac{d-1}{2} \max_{2 \le j \le d} |\theta^*_1 - \theta^*_j|
\le d \, \|\theta^*\|_\infty
$$
and
$$
\E[Z_r^2] = \frac{(d-1)^2}{4} \E\bigg[ \sum_{j=2}^d (\theta^*_1 - \theta^*_j)^2 \bbone \{ x_r = e_1 - e_j \} \bigg]
= \frac{(d-1)^2}{4} \sum_{j=2}^d \frac{2 (\theta^*_1 - \theta^*_j)^2}{d(d-1)}
\le 2 d \, \|\theta^*\|_\infty^2 .
$$
Bernstein's inequality then yields the desired bound.
%implies that
%$$
%\bigg| \frac 1N \sum_{r=1}^N Z_ r - \theta^*_1 \bigg|
%\le C \Big( \sqrt{\frac{d}{N}} \|\theta^*\|_\infty \sqrt{\log \frac{1}{\delta}} + \frac{d}{N} \|\theta^*\|_\infty \log \frac{1}{\delta} \Big)
%$$
%with probability at least $1 - \delta$, which completes the proof.
\end{proof}


\begin{lemma}
\label{lem:eps-r-conc}
Suppose that $(x_r)_{r=1}^N$ are i.i.d.\ from the uniform distribution over $\{ e_i - e_j : (i,j) \in \binom{[d]}{2} \}$, and that $(\eps_r)_{r=1}^N$ are independent $\subG(\sigma^2)$ random variables.
Then there are absolute constants $C, c > 0$ such that for any $\delta \in (0,1)$, it holds with probability at least $1 - \delta - \exp(-cN/d)$ that
$$
\bigg| \sum_{r = 1}^N \sum_{j=2}^d \eps_r \, \bbone \{ x_r = e_1 - e_j \} \bigg|
\le C \sigma \sqrt{\frac{N}{d} \log \frac{1}{\delta}}  .
$$
\end{lemma}

\begin{proof}
Let $N_1 = \sum_{r = 1}^N \sum_{j=2}^d \bbone \{ x_r = e_1 - e_j \}$.
Then we have $N_1 \sim \Bin(N, 2/d)$.
By a standard binomial tail bound, we get
%$N_1 \le C_1 \big( \sqrt{\frac{N}{d} \log \frac{1}{\delta}} + \log \frac{1}{\delta} \big)$
%with probability at least $1 - \delta$ for an absolute constant $C_1>0$.
$N_1 \le 4 N/d$
with probability at least $1 - \exp(- c N/d)$ for an absolute constant $c>0$.
Furthermore, conditional on $N_1$, we have
$\sum_{r = 1}^N \sum_{j=2}^d \eps_r \, \bbone \{ x_r = e_1 - e_j \} \sim \subG(\sigma^2 N_1)$.
As a result,
$$
\bigg| \sum_{r = 1}^N \sum_{j=2}^d \eps_r \, \bbone \{ x_r = e_1 - e_j \} \bigg|
\le C_2 \sigma \sqrt{N_1 \log \frac{1}{\delta}}
$$
with probability at least $1 - \delta$ conditional on $N_1$ for an absolute constant $C_2>0$.
Combining this with the bound on $N_1$ finishes the proof.
\end{proof}

\end{comment}


